Diagnostic Benchmark and Iterative Inpainting for Layout-Guided Image Generation

Spatial control is a core capability in controllable image generation. Advancements in layout-guided image generation have shown promising results on in-distribution (ID) datasets with similar spatial configurations. However, it is unclear how these models perform when facing out-of-distribution (OOD) samples with arbitrary, unseen layouts. In this paper, we propose LayoutBench, a diagnostic benchmark for layout-guided image generation that examines four categories of spatial control skills: number, position, size, and shape. We benchmark two recent representative layout-guided image generation methods and observe that the good ID layout control may not generalize well to arbitrary layouts in the wild (e.g., objects at the boundary). Next, we propose IterInpaint, a new baseline that generates foreground and background regions step-by-step via inpainting, demonstrating stronger generalizability than existing models on OOD layouts in LayoutBench. We perform quantitative and qualitative evaluation and fine-grained analysis on the four LayoutBench skills to pinpoint the weaknesses of existing models. We show comprehensive ablation studies on IterInpaint, including training task ratio, crop&paste vs. repaint, and generation order. Lastly, we evaluate the zero-shot performance of different pretrained layout-guided image generation models on LayoutBench-COCO, our new benchmark for OOD layouts with real objects, where our IterInpaint consistently outperforms SOTA baselines in all four splits. Project website: https://layoutbench.github.io

==> images/intermediate_steps_example_additional.tex <==
\begin{table*}[t]
\begin{center}
    \resizebox{\linewidth}{!}{
      
        \begin{tabular}{l | c c c c c c c c c c c c c | c}
          \toprule

      
          Update & \multicolumn{13}{c |}{{\large  Intermediate Generation}}
          & {\large  GT image} \\
          \midrule

        & Step 1 & Step 2 & Step 3 & Step 4 & Step 5 & Step 6 & Step 7 & Step 8 & Step 9 & Step 10 & Step 11 & Step 12 & Step 13 \\
            Prompts & 
            Add red metal cube &
            Add purple metal sphere &
            Add cyan metal cube &
            Add gray metal cube &
            Add brown rubber cube &
            Add blue rubber cube &
            Add purple rubber cube &
            Add purple metal cube &
            Add gray metal cylinder &
            Add yellow rubber cylinder &
            Add gray rubber cylinder &
            Add red rubber cylinder &
            Add gray background \\
          \midrule
        \makecell[l]{Crop\&Paste \\ (default)}
          & \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/LayoutBench_val_number_11-13_001680/0_generated.png}} &
          \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/LayoutBench_val_number_11-13_001680/1_generated.png}} &
          \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/LayoutBench_val_number_11-13_001680/2_generated.png}} &
          \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/LayoutBench_val_number_11-13_001680/3_generated.png}} &
          \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/LayoutBench_val_number_11-13_001680/4_generated.png}} &
          \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/LayoutBench_val_number_11-13_001680/5_generated.png}} &
          \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/LayoutBench_val_number_11-13_001680/6_generated.png}} &
          \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/LayoutBench_val_number_11-13_001680/7_generated.png}} &
          \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/LayoutBench_val_number_11-13_001680/8_generated.png}} &
          \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/LayoutBench_val_number_11-13_001680/9_generated.png}} &
          \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/LayoutBench_val_number_11-13_001680/10_generated.png}} &
          \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/LayoutBench_val_number_11-13_001680/11_generated.png}} &
          \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/LayoutBench_val_number_11-13_001680/12_generated.png}} &
          \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/LayoutBench_val_number_11-13_001680.png}} \\
          \midrule
          Repaint &
            \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/Nopaste_LayoutBench_val_number_11-13_001680/0_generated.png}} &
            \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/Nopaste_LayoutBench_val_number_11-13_001680/1_generated.png}} &
            \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/Nopaste_LayoutBench_val_number_11-13_001680/2_generated.png}} &
            \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/Nopaste_LayoutBench_val_number_11-13_001680/3_generated.png}} &
            \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/Nopaste_LayoutBench_val_number_11-13_001680/4_generated.png}} &
            \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/Nopaste_LayoutBench_val_number_11-13_001680/5_generated.png}} &
            \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/Nopaste_LayoutBench_val_number_11-13_001680/6_generated.png}} &
            \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/Nopaste_LayoutBench_val_number_11-13_001680/7_generated.png}} &
            \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/Nopaste_LayoutBench_val_number_11-13_001680/8_generated.png}} &
            \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/Nopaste_LayoutBench_val_number_11-13_001680/9_generated.png}} &
            \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/Nopaste_LayoutBench_val_number_11-13_001680/10_generated.png}} &
            \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/Nopaste_LayoutBench_val_number_11-13_001680/11_generated.png}} &
            \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/Nopaste_LayoutBench_val_number_11-13_001680/12_generated.png}} &
            \adjustbox{valign=c}{\includegraphics[height=0.1\textwidth]{images/intermediate_generation/LayoutBench_val_number_11-13_001680.png}} \\
          \bottomrule
      \end{tabular}
    }
\end{center}
\caption{
Additional intermediate generation samples of \method{}.
}
\label{tab:intermediate_generation_samples_addtional}
\end{table*}

==> tables/ablation.tex <==

\begin{table}[H]
\centering
\tablestyle{3pt}{1.1} \vspace{-2ex}
    \resizebox{\linewidth}{!}{
      \begin{tabular}{c c c c}
          \toprule
          Image Update & FG/BG Training Ratio & Generation Order & \benchmark{} AP \\
          \midrule
          
          
          Crop \& Paste & 3:7 & Random & 36.5 \\

          \midrule

          
          Repaint & & & 24.4 \textcolor{red}{(-12.1)} \\

          \midrule

          & 1:9 & & 36.0 \textcolor{red}{(-0.5)} \\
          & 5:5 & & 35.0 \textcolor{red}{(-1.5)} \\
          & 7:3 & & 34.2 \textcolor{red}{(-2.3)} \\
          & 10:0 (No BG) & & 27.5 \textcolor{red}{(-9.0)} \\

          \midrule
          
          & & Top $\rightarrow$ Bottom & 37.2 \textcolor{green}{(+0.7)} \\
          & & Bottom $\rightarrow$ Top & 36.1 \textcolor{red}{(-0.4)} \\

          \bottomrule
        \end{tabular}
    }
\caption{Ablation studies on \method{}}
\label{tab:ablation}
\end{table}

